Protoplanetary and debris disks in the $\eta$ Chamaeleontis Association: A sub-millimeter survey obtained with APEX/LABOCA

Nearby associations are ideal regions to study coeval samples of protoplanetary and debris disks down to late M-type stars. Those aged 5-10,Myrs, where most of the disk should have already dissipated forming planets, are of particular interest. We present the first complete study of both protoplanetary and debris disks in a young region, using the $\eta$ Chamaeleontis association as a test bench to study the cold disk content. We obtained sub-millimeter data for the entire core population down to late M-type stars, plus a few halo members. We performed a continuum sub-millimeter survey with APEX/LABOCA of all the core populations of $\eta$ Cha association. Disk properties have been derived by modeling protoplanetary and debris disks using RADMC 2D and DMS, respectively. We find that protoplanetary disks in $\eta$ Cha typically have holes with radii of the order of 0.01 to 0.03 AU, while ring-like emission from the debris disks is located between 20 au and 650 au from the central star. The parallaxes and Gaia eDR3 photometry, in combination with the PARSEC and COLIBRI isochrones, enable us to confirm an age of $\eta$ Cha between 7 and 9 Myrs. In general, the disk mass seems insufficient to support accretion over a long time, even for the lowest mass accretors, a clear difference compared with other regions and also a sign that the mass budget is further underestimated. We do not find a correlation between the stellar masses, accretion rates, and disk masses, although this could be due to sample issues. We confirm that the presence of inner holes is not enough to stop accretion unless accompanied by dramatic changes to the total disk mass content. Comparing $\eta$ Cha with other regions at different ages, we find that the physical processes responsible for debris disks (e.g., dust growth, dust trapping) efficiently act in less than 5 Myrs.

==> etacha_gaia.tex <==

\section{Cluster members on the {\it Gaia}/DR2}
The membership of the $\eta$ Cha cluster was first defined by the follow up spectroscopic observations of 
X-ray sources \citep{Mamajeketal1999}. Successively \citet{Murphyetal2010} looked for halo members 
 within 5.5$^\circ$ from the $\eta$ Cha cluster using optical and near-infrared photometry, astrometry (using the Naval Observatory Merged Astrometric Catalogue, NOMAD), and with a spectroscopic follow-up campaign. They found seven new probable and possible members. \\
%{\it Gaia} allows us now to look for new halo members, and confirm the previously suggested members. The power of this approach applied to nearby associations was showed by \citet{gagneetal2018}.  While in the first release of {\it Gaia}, only two $\eta$ Cha members were present, the new data release (DR2) has all the sources (besides one) with astrometric measurements, as it is shown in Table~\ref{gaia}.
While in the first release of {\it Gaia} only two sources of $\eta$ Cha were present \footnote{2MASS08414471-7902531 and 2MASS08365623-7856454}, all the cluster members, apart of one are present in the {\it Gaia}/DR2 data 
(summarized in Table~\ref{gaia}). 
We apply a maximization of the total likelihood function (MLE) of a multivariate Gaussians model, where each gaussian characterize  
the distribution of the each astrometric parameter. This approach \citep[as demonstrated by ][]{Roccatagliataetal2018, Franciosinietal2018} allows us to take into account the errors and the correlations between the parameters. 
We obtain a parallax of $\pi = 10.12\pm0.09$~mas, which corresponds to a distance of 98.8~$\pm$~0.9~pc. The proper motions are $\mu_\alpha = -29.48\pm1.10$ mas/yr; $\mu_\delta = 27.10\pm0.69$~mas/yr, in RA and DEC respectively. \\
%On a sample of 1\,634\,628 sources downloaded from the {\it Gaia} archive, 8\,354 of which with a parallax higher than 0.5 mas, excess noise lower than 1 and percentage error in parallax lower than 40$\%$, we adopt the quantitative approach presented in \citet{Roccatagliataetal2018, Franciosinietal2018} to fit the distributions of parallax and proper motions with a double 3D multivariate Gaussians model in order to disentangle the cluster from the field contribution. The best fit astrometric parameters, with their corresponding dispersions, are obtained by the maximization of the total likelihood function (MLE) of a single population of the initial cluster members (highlighted in Table\ref{gaia}). 
Figure~\ref{dss-pm} shows the proper motions of the core and the halo members, respectively, on the background an optical image of the region. The proper motions of the three halo members seem to be consistent with those of the core cluster. However, checking in detail also Table~\ref{gaia}, we notice that one of the three halo members lies at about 25 pc further away from 
RX J1005.3-7749\footnote{Gaia DR2 5202670052321415040}

{\color{red} Vero: I find this section a bit confusing (maybe because it is not done yet). I am not sure what you intend to do with the 2nd paragraph. Study the cluster properties and whether they are different groups, etc?}


\subsection{Archival FEROS data}

%{\color{red} Do we want to put the info on the SED here too?}
To complete the kinematic picture obtained from the Gaia data, we also use archival high-resolution spectroscopy to obtain additional and more precise radial velocity measurements. The available spectroscopy was obtained with the ESO/MPG 2.2m telescope using the FEROS instrument \citep{kaufer99}, which provides coverage between 340-920 nm with a spectral resolution 48,000. Several of the $\eta$ Cha members (RECX-1, RECX-3, RECX-4, RECX-6, RECX-10, RECX-12, $\eta$ Cha, HD75505, and RS Cha) have been observed with FEROS as part of program 084.A-9003 (PI J. Setiawan) and 082.A-9008 (PI V. Roccatagliata). The data were obtained from the ESO science archive, and have been reduced by the FEROS automated pipeline {\color{red} and then corrected to remove the offset in the barycentric velocity for the FEROS spectra \citep{Mulleretal2013} RIGHT?}. For most of the objects, repeated observations exists, so that we selected those that have the best S/N (typically, between 50 and 300). 

For the late-type objects, we selected the regions of the spectra between 5200-5800$\AA$ and 5400-600$\AA$, which do not contain significant activity-related or telluric
lines \citep{curcio64} and measured the rotational and radial velocity by 
cross-correlating the object spectra with two rotational standards \footnote{Taken from: http://obswww.unige.ch/\%7Eudry/std/stdnew.dat} observed with the same resolution by FEROS, HD 115414 (spetral type K2) and HD 125184 (G5). For the massive ones, we use the templates HD 193432 (B9.5) and HD 27962 \citep[A2;][]{fekel99} and the spectral region between 4200-6700$\AA$. For all objects, we used
PyAstronomy task $rotBroad$ to create artificially broadened templates, and  $crosscorRV$ to obtain the cross-correlation. Note that RS-Cha is a known spectroscopic binary, so it cannot be used for our purposes, and $\eta$ Cha and HD 75505 give ambiguous results that suggests they may have radial velocity variability (as most early-type stars), so at the end they cannot be used for our purposes.
The resulting radial velocities are listed in Table \ref{gaia}.


\begin{small}
\begin{table*}
\caption{Parallaxes,proper motions and radial velocity from {\it Gaia} DR2. For some objects we include the spectroscopic radial velocity (marked with $^s$). }
\label{gaia}      
\centering               
\begin{tabular}{rr rr r r r}  
\hline\hline                
\noalign{\smallskip}
source&2MASSJ & $\pi$ [mas] &  d [pc] & $\mu_\alpha$ [mas/yr] & $\mu_\delta$ [mas/yr] &RV [km/s]\\
\noalign{\smallskip}
\hline                .
\noalign{\smallskip}
 $\eta$ Cha	&	08411947-7857481		&	10.04	$\pm$	0.09	&	99.56	$\pm$	0.90	&	-29.78	$\pm$	0.22	&	26.60	$\pm$	0.25	&	53:$^s$			\\
RS Cha	&	08431222-7904123		&	10.10	$\pm$	0.04	&	99.05	$\pm$	0.38	&	-27.17	$\pm$	0.07	&	28.02	$\pm$	0.07	&	Spec. Binary			\\
HD 75505	&	08414471-7902531		&	10.00	$\pm$	0.03	&	100.01	$\pm$	0.33	&	-30.75	$\pm$	0.06	&	27.04	$\pm$	0.08	&				\\
J0836	&	08361072-7908183		&	10.15	$\pm$	0.09	&	98.50	$\pm$	0.87	&	-28.62	$\pm$	0.14	&	28.03	$\pm$	0.16	&				\\
J0838	&	08385150-7916136		&	9.96	$\pm$	0.09	&	100.42	$\pm$	0.87	&	-28.49	$\pm$	0.15	&	26.62	$\pm$	0.19	&				\\
J0841	&	08413030-7853064		&	10.12	$\pm$	0.06	&	98.81	$\pm$	0.59	&	-30.25	$\pm$	0.12	&	28.23	$\pm$	0.14	&				\\
J0843	&	08431857-7905181		&	10.91	$\pm$	0.31	&	91.67	$\pm$	2.63	&	-27.34	$\pm$	0.49	&	27.32	$\pm$	0.57	&				\\
J0844	&	08440914-7833457		&	10.15	$\pm$	0.08	&	98.48	$\pm$	0.80	&	-29.54	$\pm$	0.14	&	26.23	$\pm$	0.15	&				\\
RECX-1	&	08365623-7856454		&	9.98	$\pm$	0.13	&	100.16	$\pm$	1.27	&	-29.64	$\pm$	0.25	&	27.57	$\pm$	0.22	&	17.58	$\pm$	1.37;  18.1$\pm$0.2$^s$	\\
RECX-3	&	08413703-7903304		&	10.12	$\pm$	0.04	&	98.81	$\pm$	0.36	&	-28.59	$\pm$	0.06	&	27.42	$\pm$	0.09	&	17.85$\pm$0.25$^s$			\\
RECX-4	&	08422372-7904030		&	10.05	$\pm$	0.02	&	99.53	$\pm$	0.23	&	-30.86	$\pm$	0.04	&	25.88	$\pm$	0.05	&	16.01	$\pm$	1.21; 18.05$\pm$0.15$^s$	\\
RECX-5	&	08422710-7857479		&	10.12	$\pm$	0.05	&	98.77	$\pm$	0.44	&	-30.30	$\pm$	0.08	&	27.25	$\pm$	0.09	&				\\
RECX-6	&	08423879-7854427		&	10.19	$\pm$	0.04	&	98.12	$\pm$	0.40	&	-29.16	$\pm$	0.07	&	27.01	$\pm$	0.08	&	17.8$\pm$0.3$^s$			\\
RECX-7	&	08430723-7904524		&	10.13	$\pm$	0.02	&	98.74	$\pm$	0.23	&	-30.18	$\pm$	0.04	&	27.45	$\pm$	0.04	&				\\
RECX-9	&	08441637-7859080		&				&				&				&				&				\\
RECX-10	&	08443188-7846311		&	10.19	$\pm$	0.03	&	98.18	$\pm$	0.30	&	-30.30	$\pm$	0.06	&	26.86	$\pm$	0.05	&	17.70$\pm$0.05$^s$			\\
RECX-11	&	08470165-7859345		&	10.14	$\pm$	0.03	&	98.58	$\pm$	0.25	&	-30.12	$\pm$	0.05	&	26.68	$\pm$	0.04	&				\\
RECX-12	&	08475676-7854532		&	10.45	$\pm$	0.07	&	95.67	$\pm$	0.60	&	-30.14	$\pm$	0.12	&	26.51	$\pm$	0.12	&	11.95$\pm$0.05$^s$			\\ \noalign{\smallskip}
RX J1005.3-7749	&	10052006-7748423		&	9.97	$\pm$	0.02	&	100.34	$\pm$	0.22	&	-37.4	$\pm$	0.04	&	14.62	$\pm$	0.04	&	12.06	$\pm$	3	\\
J0801	&	08014860-8058052		&	8.88	$\pm$	0.05	&	112.57	$\pm$	0.64	&	-18.79	$\pm$	0.09	&	28.98	$\pm$	0.11	&				\\
J0820	&	08202975-8003259		&	10.30	$\pm$	0.06	&	97.05	$\pm$	0.53	&	-27.66	$\pm$	0.09	&	29.50	$\pm$	0.13	&				\\
\hline                        
\noalign{\smallskip}
\end{tabular}
%L04: \citet{Lawsonetal2004}; 
%M11: \citet{Murphyetal2013}; 
%M13: \citet{Murphyetal2011}; 
%SA09: \citet{Sicilia-Aguilaretal2009}.
\end{table*}
\end{small}



\begin{figure*}
\centering
\begin{tabular}{cc}
\includegraphics[width=0.9\linewidth]{fig/etacha_dss_pm.jpg}
\end{tabular}
\caption{DSS optical view of the $\eta$ Chamaeleon region. The arrows represent the proper motions of each source. The green and cyan arrows represent the core and the halo members, respectively. 10$''$ arrow corresponds to a proper motion of 1mas/yr. \label{dss-pm}}
\end{figure*}



Can we connect what we observe with the cluster structure? For instance, distinguish groups of stars 
according to their formation and see if this makes sense with their disks and whether it may also
explain potential differences in star formation and disk evolution between sparse and dense clusters 
(e.g. Hsu et al. 2013, Fang et al. 2013), or disk survival vs environment.. 

{\color{magenta} Some ideas looking at the Gaia table and RV:\\
For the main cluster members, it looks like the differences in PM and RV are very small. For the PM I 
see up to 2-3 mas/yr maximum offset in each direction, rv also quite similar for the objects with 
similar parallax and PM (curiously, RECX-12 has a larger RV offset but also a different parallax... 
although some sources may also be undetected binaries). 2-3 mas/yr means about 1-1.4 km/s. 1km/s means 
that the star will cover 1 pc in 1 Myr. This is something to consider for a cluster that is $>$6 Myr. 
If all these stars are still clustered, it means they have formed with nearly zero velocities with 
respect to each other. This seems to agree with the data, but typical velocity ranges in clouds are 
larger.\\
We may be able to statistically tell something about the forming conditions. Or why some other members 
have been missing. Can we check if there are any signs of converging velocities (plotting them as
relative velocities), such as what we see for the Tr37 filament, or anything that may indicate that the stars have formed as part of a subcluster or grouplet or by gravitational focusing or similar? That is, can we tell whether it is likely that these objects formed as totally independent protostars, or not? From the Bate simulations, it looks to me that any highly interactive cluster would tend to kick them out a lot faster than what is observed. }

